A Microbenchmark Characterization of the Emu Chick

The Emu Chick is a prototype system designed around the concept of migratory memory-side processing. Rather than transferring large amounts of data across power-hungry, high-latency interconnects, the Emu Chick moves lightweight thread contexts to near-memory cores before the beginning of each memory read. The current prototype hardware uses FPGAs to implement cache-less "Gossamer cores for doing computational work and a stationary core to run basic operating system functions and migrate threads between nodes. In this multi-node characterization of the Emu Chick, we extend an earlier single-node investigation (Hein, et al. AsHES 2018) of the the memory bandwidth characteristics of the system through benchmarks like STREAM, pointer chasing, and sparse matrix-vector multiplication. We compare the Emu Chick hardware to architectural simulation and an Intel Xeon-based platform. Our results demonstrate that for many basic operations the Emu Chick can use available memory bandwidth more efficiently than a more traditional, cache-based architecture although bandwidth usage suffers for computationally intensive workloads like SpMV. Moreover, the Emu Chick provides stable, predictable performance with up to 65% of the peak bandwidth utilization on a random-access pointer chasing benchmark with weak locality.

==> sections/highlights.tex <==
\textbf{Highlights of this work}

This study evaluates multi-node performance of microbenchmarks including STREAM, pointer chasing, and SpMV on the Emu Chick prototype. It demonstrates that the peak STREAM bandwidth of the Emu system is 12 GB/s and that pointer chasing can attain up to 65\% of this peak bandwidth. Remote recursive spawn is determined to be the best spawn strategy for the Chick, and 2D layout is shown to be best for SpMV with a peak performance of 6 GB/s for synthetic graphs.

\newpage
\newpage
